Clinician-in-the-Loop Decision Making: Reinforcement Learning with Near-Optimal Set-Valued Policies

Standard reinforcement learning (RL) aims to find an optimal policy that identifies the best action for each state. However, in healthcare settings, many actions may be near-equivalent with respect to the reward (e.g., survival). We consider an alternative objective -- learning set-valued policies to capture near-equivalent actions that lead to similar cumulative rewards. We propose a model-free algorithm based on temporal difference learning and a near-greedy heuristic for action selection. We analyze the theoretical properties of the proposed algorithm, providing optimality guarantees and demonstrate our approach on simulated environments and a real clinical task. Empirically, the proposed algorithm exhibits good convergence properties and discovers meaningful near-equivalent actions. Our work provides theoretical, as well as practical, foundations for clinician/human-in-the-loop decision making, in which humans (e.g., clinicians, patients) can incorporate additional knowledge (e.g., side effects, patient preference) when selecting among near-equivalent actions.

==> backup.tex <==
In \cref{fig:mimic-plots} we show the training curves as the algorithm converges.

\begin{figure}[h]
\begin{subfigure}[b]{.48\linewidth}
\centering \includegraphics[width=\linewidth]{updated/mimic-training_curve.png}
\caption{Q-values stabilize as training progresses (quartiles of $Q(s,a)$ shown)}\label{fig:mimic-train}
\end{subfigure}%
\quad
\begin{subfigure}[b]{.46\linewidth}
\centering \includegraphics[width=\linewidth]{fig_mimic/mimic-td_error.pdf}
\caption{TD error decreases and remains bounded as training progresses. }\label{fig:mimic-td}
\end{subfigure}
\caption{Training curves for the near-greedy TD algorithm on \textsf{MIMIC-sepsis} with $\zeta=0.05$.}\label{fig:mimic-plots}
\end{figure}


%Future work can extend our approach by relaxing the action selection strategies or incorporating policy-based methods. 

% in a TD learning framework, we effectively constrain the form of the target policy, resulting in a TD-style algorithm . 
% for the near-greedy heuristic, we modify the update rule in Q-learning as shown in \cref{alg:near-greedy}. 
% The conservative version is similar, except line 8 is replaced with the conservative heuristic in \cref{eqn:conservative}, and the output step adjusted accordingly. 
% The algorithm is a relaxed version of Q-learning, alternating between policy evaluation and policy improvement. For policy improvement, instead of selecting actions greedily with respect to Q-values, we use the near-greedy heuristic. Compared to Q-learning, which updates $Q(s,a)$ based on greedy action selection for the next state $s'$, we temporarily construct a candidate SVP for the next state $s'$ using the current estimates of the Q-values (line 8). In cases where $\pi(s') = \varnothing$ is empty (due to zero initialization of Q-values) or $V^*(s)<0$, the algorithm reverts back to greedy policy construction (line 12). 


% \citep{watkins1992q,melo2001convergence,van2009expectedSARSA}: sufficient exploration and appropriately decayed step size $\alpha$. 
%More precisely, each $(s,a)$ is updated infinitely many times, $\sum_{t} \alpha_{t}=\infty$, and $\sum_{t} \alpha_{t}^{2}<\infty$. 

% For a general MDP, such a near-greedy SVP may not exist due to the recursive dependence between $\pi$ and $Q^{\pi}$. Specifically, it is possible that: i) not including an action $a$ in $\pi(s)$ violates the near-greedy heuristic as $Q(s,a) \geq (1-\zeta)V^{*}(s)$, and ii) including the action $a$ in $\pi(s)$ decreases the value function $Q(s,a)$ to be $<(1-\zeta)V^{*}(s)$ such that $a$ is no longer near-optimal (see \cref{appx:non-existence} for an example). Moreover, in the near-greedy TD algorithm, the update operator is not a contraction in general (\cref{appx:contraction}), and thus the algorithm is not guaranteed to converge. However, existence of near-greedy SVPs and convergence guarantees can be established under certain conditions. 


% Let $a^* = \argmax_{a\in \mathcal{A}} Q^{*}(s,a)$ such that $V^*(s) = Q^*(s,a^*)$, then:
% \begin{align*} \small
%     Q^{\pi}(s,a^*) &= r(s,a^*) + \gamma \mathbb{E}_{s'|s,a^*} V^{\pi}(s') \\
%     &\geq r(s,a^*) + \gamma \mathbb{E}_{s'|s,a^*} (1-\zeta) V^{*}(s') \\
%     &= \zeta r(s,a^*) + (1-\zeta) [r(s,a) + \gamma \mathbb{E}_{s'|s,a^*} V^{*}(s')] \\
%     &= \zeta r(s,a^*) + (1-\zeta) Q^{*}(s,a^*) \\
%     &\geq (1-\zeta) V^{*}(s) .
% \end{align*}
%
% To see this, let $a^* = \argmax_{a\in \mathcal{A}} Q^{*}(s,a)$ such that $V^*(s) = Q^*(s,a^*)$. Then, 
% \begin{align*}
%     Q^{\pi}(s,a^*) &\geq \zeta r(s,a^*) + (1-\zeta) Q^{*}(s,a^*) \\
%     &= \zeta r(s,a^*) + (1-\zeta) V^{*}(s) \\
%     &\geq (1-\zeta) V^{*}(s)
% \end{align*}


% choosing an appropriate regularization weight and a probability threshold. In practice, these hyperparameters can be difficult to determine without knowledge of the learned action distributions, and they do not correspond to the near-optimality constraint. 

% Since these two MDPs do not have stochastic transitions or stochastic rewards, the algorithm reduces to fixed-point iteration, when using a constant step size of $\alpha=1$, and the temporal-difference (TD) error should eventually go to $0$ if a fixed-point exists. We monitor the TD error towards the end of learning, running the algorithm for the same number of iterations in which Q-learning would converge (where TD error is effectively zero). 


% For illustrative purposes, we focus on $\zeta=0.025$. On the test set, the estimated return following $\pi$ is within $\sim 3\%$ of the estimated optimal return. To understand the relationship among actions, for each action we count the number of times every other action is suggested by the learned SVP as near-equivalent. These counts are aggregated over all states in the test set, and normalized by the maximum count (\cref{fig:mimic_actions}). We focus on actions that occur together $>80\%$ of the time, i.e., actions considered near-equivalent for most states.\\ 

% The bottom row corresponds to actions with no IV fluids and some amount of vasopressors. These actions appear to be near-equivalent to treatments with no vasopressors, but high doses of IV fluids. These near-equivalencies indicate alternative treatment options that are expected to lead to similar outcomes. 


%A more in-depth analysis might consider near-equivalency at the state-level.% However, given the size of the state space this proved challenging. 

% The current near-greedy formulation acts equally greedily for each state, possibly leading to non-convergence in a non-DAG environment. Future work might consider alternatives to adjusting the action selection strategy. Besides annealing the step size so that changes in Q-values are negligible towards the end of training, one could perform an alternating minimization procedure that more clearly delineates policy improvement and policy evaluation, or a mixing/switching of the two action selection strategies, to better adapt to the problem. 

% Our approach can be readily extended to problems with continuous state space (via function approximators for the Q-function) \citep{mnih2015human, raghu2017deepRL}, and can be combined with other extensions of TD-learning \citep{hasselt2010double, wang2015dueling}, or used as components of an actor-critic framework \citep{konda2000actor}. 
% comparable to Q-learning in terms of sample efficiency
% a complementary valued-based approach and could be combined with these policy-based methods.

%Future work can apply our approach to clinical settings with more complex action structures, and provide more meaningful alternative treatment recommendations. 
% The proposed approach can be augmented with other improvements for value-based methods \citep{hasselt2010double, wang2015dueling, mnih2015human}, as well as incorporated into policy-based methods \citep{konda2000actor}, 

%we identified subsets of states as `healthiest 10\%' and `sickest 10\%' by considering states with the highest and lowest survival probability, as predicted by a model learned from the training set. especially in the region of actions with low-to-moderate IV/vasopressor doses. 

%Occasionally, we observe near-equivalency between large vasopressor and large fluid doses (bottom right cell). 

% In these extreme circumstances, these actions are learned from patients In such scenarios, clinicians may choose to do nothing or do everything, resulting in this particular combination of actions in the allowable action space for the RL agent. 

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.6\linewidth]{updated/{Vstar_hist}.pdf}
%     \caption{Distribution of $V^*(s)$ values. }
%     \label{fig:mimic-values}
% \end{figure}



% We focus on actions that occur together $>60\%$ of the time, i.e., actions considered near-equivalent for most states.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{fig_mimic/{mimic-action_zeta=0.025}.pdf}
%     \caption{Near-equivalent relationships among actions in SVPs on the \textsf{MIMIC-sepsis} task with $\zeta=0.025$. Both the outer grid and the inner grid contain the 25 actions, corresponding to 5 levels of vasopressor doses and 5 levels of IV fluids. Red numbers indicate the frequency that each action is recommended. }
%     \label{fig:mimic_actions}
% \end{figure}

% \begin{figure}[ht!]
% \begin{subfigure}[b]{.45\linewidth}
% \centering \includegraphics[width=0.82\linewidth, trim=0 0 75 0, clip]{updated/{mimic-action_zeta=0.05_sickest}.pdf}
% \caption{Sickest 10\% states.}\label{fig:mimic-train}
% \end{subfigure}%
% \quad
% \begin{subfigure}[b]{.45\linewidth}
% \centering \includegraphics[width=\linewidth]{updated/{mimic-action_zeta=0.05_healthiest}.pdf}
% \caption{Healthiest 10\% states.}\label{fig:mimic-td}
% \end{subfigure}
% \caption{Action equivalences for sickest vs. healthiest states in the test set. }\label{fig:sick-healthy}
% \end{figure}


% \begin{figure}[ht]
% \begin{subfigure}[b]{.45\linewidth}
% \centering \includegraphics[width=\linewidth]{updated/{Vstar_hist}.pdf}
% \caption{}\label{fig:mimic-values}
% \end{subfigure}%
% \quad
% \begin{subfigure}[b]{.45\linewidth}
% \centering \includegraphics[width=\linewidth]{updated/{Vstar_psize}.pdf}
% \caption{}\label{fig:mimic-psize}
% \end{subfigure}
% \caption{(a) Distribution of $V^*(s)$ (values $<80$ are not shown). (b) Average size of $\pi(s)$ for states with different $V^*(s)$ values (grouped into quartiles). }\label{fig:}
% \end{figure}


% \subsection*{Extensions to continuous state space}
% Our proposed algorithms follow the TD learning framework and use gradient-like update rules. Thus it is straightforward to extend the Q-table setting to function approximator of Q (a regressor such as a neural network). Specifically, assuming the Q function is parametrized by $Q(s,a; \mathbf{w})$, then the update on line 10 of \cref{alg:near-greedy} would change to the following: 
% \begin{align*}
%     \mathbf{w} \leftarrow \mathbf{w}+\alpha\Big[ r + \gamma \min _{a'\in\pi(s')} &Q(s', a'; \mathbf{w}) \\
%     & \left. - Q(s, a; \mathbf{w})\right] \nabla_{\mathbf{w}} Q(s, a; \mathbf{w})
% \end{align*}

% This adaptation is certainly feasible, but any convergence guarantees would be lost as there is no notion of a DAG in a continuous state space. With appropriate settings of $\zeta$ and proper training procedures similar to deep Q-learning, we expect the algorithm to learn meaningful policies.

